The Probabilistic Analysis of the Communication Network created by Dynamic Boundary Coverage

We do a Probabilistic Analysis of the Network generated by robots involved in Stochastic Boundary Coverage

==> Applications.tex <==
\section{Applications}
\label{Sec:Applications} 

\subsection{Recruitment until saturation}

Thus far, we considered problem instances $Q$ that had a fixed number of robots. Suppose now that we are presented with problem instances at every instant of time, in which we are asked to compute $\psat$, $\favn$, or the marginal pdf of order statistics. It is easy to see that computing marginal pdfs, etc. is $\PH$ at every time instant. We state this result immediately in the following theorem.

\begin{theorem}
\label{th:time} 
 Suppose that each robot attaches to the boundary uniformly with probability $p_b$ at every time instant, or detaches from the boundary with probability $p_u$ attached. Then it is $\PH$ to compute $\psat$ and $f_{\rvsvec_{\ixs}}$ under saturation every time instant. 
 \end{theorem}

 
We may apply \autoref{th:time} to our previous work. 
\begin{enumerate}
 \item In \cite{KumarSHS2013}, we model collective transport in ants using a stochastic hybrid system (SHS). The behavioural part of the SHS consists of a 3-state PFSM in which ants attach to the back of the load, to its front, or remain detached. Since the PFSM in \autoref{th:time} is a simplified version of the ant model, it follows that saturation queries on the 3-state PFSM would be $\PH$ at every time instant.
 \item In \cite{PavlicISRR2013, WilsonSwarmInt2014}, we model robots binding and unbinding from a boundary with probabilities $p_b e_u$ and $p_u e_b$. The statement of \autoref{th:time} applies here as well. \todo{continuous-time attachments/detachments}?
 \end{enumerate}



\subsection{Parking Problem}

The above results immediately generalize to the problem of \textit{collision-permissive attachments}. Here a team of robots each of which has radius $\rad$, attaches to the boundary in such a way that the disk of each robot falls within the boundary, and robots can possibly collide with each other. In other words, robots are collectively attaching to a boundary of total length $s + \dia$. All previous results remain intact, if we think of $\pos{i}$ as the midpoint of robot $i$.

We define the \textit{$n$-robot parking variant} as a problem in which there are no collisions among the $\nor$ robots attach. Unlike in \textit{Renyi Parking}, where robots attach until saturation, here the number of attached robots is always $\nor$. As before, let $\pos{i}$ be the midpoint of the $i$-th robot. The distance between every pair of robot positions is then at least $\dia$. Then every parked configuration has a slack vector $\svec$ constrained by 
\begin{align}
\label{eqn:park1}
0\leq \svec -\dia 1^T   ,~ \1^T \svec = s , ~
\end{align}

Define the length of the unoccupied boundary between two adjacent robots to be the free slack $\fsi{i} : = \si{i} - \dia$, and the total unoccupied space to be the total free slack $\fsla$. Then we may rewrite  \autoref{eqn:park1} as
\begin{align}
 0\leq \fsvec , ~ \1^T \fsvec = \fsla
\end{align}

We call the corresponding slack simplex the free slack simplex $\fsimpn$. Given a saturating distance between the midpoints of adjacent cars, define a corresponding reduced saturating distance to be $\rsat = d - \dia$. Then every saturated configuration will have $\fsvec \leq \1^T \rsat$, and will be uniformly distributed over $\rfavn$.
This formulation is analogous to the point robots case, with the reduced / free quantities substituted for their original counterparts. Thus, all results from the previous section carry over to this problem. In particular, it is $\PH$ to evaluate the joint order statistics of a saturated configuration. 

We will now consider a variable number of cars, that park without collisions, in such a way that their mean number is $\Exp{n} = \mu$ and $\Var{n} = \sigma^2$, which is distributed on the interval $[0,\nmax]$, where $\nmax := \lfloor s/ \dia \rfloor$ is the maximum number of robots that could fit in.  This is a second order approximation to Renyi's parking problem.   To compute $\psat$, we need to have a weighted average of $\psat$ from the distribution on $[0,\nmax]$.  It is easy to see by applying an ensemble-variant of \autoref{th:time} that computing marginal pdfs is $\PH$, as is $\psat$. 






\todo{This seems suspiciously similar to slack-attach, except that we do not specify the algorithm behind parking. Is there any more precise difference?}



\subsection{Nonuniform RSA}

\subsection{Targeted Drug Delivery}

\subsection{Flocking} 


==> Exper.tex <==
\section{Experiments}
\label{Sec:Exper}
We now detail a set of computations illustrating and validating the results of previous sections. The source code for these computations is provided online in a GitLab repository \cite{polytope-comps}. 

\subsection{IID Parents}
We will deal with four parents defined on the boundary unit interval $\Bo = [0,1]$, with $s=1$: Uniform, 2-PWU , Triangular with mode at $m \in \Bo$, Beta with parameters $(a,b) \in \N$,  

\subsubsection{Instance 1}: $(d=0.4, n=2)$
The connected $\favn$ is easily found to be the equilateral triangle with vertices at the three permutations of $\begin{bmatrix} d & d & 1-2d \end{bmatrix} = \begin{bmatrix} 0.4 & 0.4 & 0.2 \end{bmatrix}$.





\subsubsection{Instance 2}: $(d=0.6, n = 2)$



\subsection{Attachment until Connectivity}



\subsection{Renyi Parking}



\subsection{Noisy Attachments}


==> Hetero.tex <==
\section{Heterogeneous Robots}
\label{Sec:Hetro}
We now consider a \textit{Heterogeneous} robot team whose Wifi adapters have different transmission power, so that $\Rob_{i}$ has connectivity threshold $d_i$. 
We call $\Rob_i$ \textit{weaker} (resp. \textit{stronger}) than $\Rob_j$ iff $\coni{i} < \coni{j}$ (resp. $\coni{i} > \coni{j}$. If $\coni{i} = \coni{j}$ we say that the two robots have equal power. Then the robot network is represented by the digraph $\G$, whose directed  edges are of the form $i \rightarrow j$ iff  $\Rob_{i}$ can transmit to $\Rob_{j}$. In general, edges are not bidirectional, for a weaker robot will not sense a stronger one, even though the converse might hold true. We find the Heterogeneous variant of $\PSAT$ to be harder than its original counterpart, by applying results from the literature on polytope volume computation.

\label{Sec:Hetero}
\subsection{Hardness of $\PSAT$}
Define the heterogeneous analogue of $\PSAT$:
\begin{align}
\label{prob:psathet}
 && \PSAT(\fpar = \Uni,s,n,\coni{1,\ldots,n}) \mapsto \pcon \nonumber \\
\text{Inputs}&:& \text{Parameters of SCS }~   s,d_i \in \Q_+ ; n \in \N \nonumber \\
\text{Output}&:&~ \text{Probability of connectivity}~ \pcon \in \Q_+  
\end{align}

\begin{theorem}
$\PSAT$ is $\PH$. 
\end{theorem}


\begin{proof}

As with homogeneous robots, the slack vector $\svec_{1:n}$ defines the simplex $\ssimpn$ in $\R^n$.  Suppose without losing generality that $d_{i}\leq d_{i+1}$, so that a connected vector requires that $\svec_{1:n}$ be nondecreasing,  leading to the constraints:
\begin{align}
\label{eqn:cuboid}
 \0 \leq \svec_{1:n} \leq d_{1:n}, ~\text{with} ~ \1^T \svec_{1:n} \leq s.  
\end{align}

We will not constrain the length of the last slack $\si{n+1}$, and thereby not prescribe connectivity there. \autoref{eqn:cuboid} stipulates that connected slack vectors lie within the hypercuboid $ \hypn:= \prod \limits _{i=1} ^{n} [0,a_i]$. Now rescale the slack coordinates $\si{i}' := \frac{\si{i}} {d_i}$ so that in the rescaled space, we have 

\begin{align}
\0 \leq \svec_{1:n}' \leq \1, ~ \text{with}~ \mathbf{d}^T \svec' \leq s.    
\end{align}

The rescaled $\favn'$ is the intersection of a cube with a half-space, and $\Vol(\favn')$ may be computed using \autoref{th:df}. Our final step is the hardness of computing $\Vol(\favn')$ \cite{DyerFrieze, dyer1991computing}: 

\begin{lemma}
\label{th:vhsp}
Define the problem $\VHSP$, which asks to find the volume of intersection between a rational half-space 
$\mathcal{T}$ (as in \autoref{eqn:hsp}, but with rational values for $\mathbf{a} $ and $b$)  and the unit hypercube, $\Vol(\mathcal{T} \cap \mathcal{C})$. $\VHSP$ is $\PH$, and has the value:

\begin{align}
 \Vol(\mathcal{T} \cap \canhyp )= n! \prod \limits_{i=1}^{n} \sum _{\vvec \in [0,1]^n} (-1)^ {\1^T \vvec} \max( (b-\avec ^T \mathbf{s})^n , 0). 
\end{align}


Equivalently, it is $\PH$ to compute the probability that a uniformly random point within $\mathcal{C}_n$ satisfies a single linear inequality. 
\end{lemma}
\end{proof}



We immediately have the result that
\begin{corollary}
Computing each of the following quantities is $\PH$:  $\Vol(\favn)$, $\Vol(\unfavn)$, and $\vm(\favn)$ for uniform parents.
\end{corollary}

\subsection{Discussion}
With homogeneous robots, $\favn$ was more symmetric compared to its heterogeneous counterpart. Exploiting this symmetry led to relatively short formulae for $\psat$ and the like. On the other hand a heterogeneous swarm is sufficiently diverse that its connected region  be an arbitrary half-space. We pay for this expressiveness by making the  connectivity problems harder. Computing $\pcon$ has a Fully Polynomial Randomized Approximation Scheme (FPRAS), which samples a uniform pdf over a subset of $\favn$ in $\Poly$,  using the Markov Chain Monte Carlo (MCMC) method \cite{JerrumCount}. Combining MCMC with Inverse CDF Sampling enables us to sample arbitrary IID pdfs over $\favn$. This approach is sufficiently general that it adapts to arbitrary joint pdfs over $\favn$, in which case it becomes the Meteropolis-Hastings sampling \cite{chib1995understanding}.    

==> IID-LB.tex <==
\subsection{Complexity of Exact Computation of $\pcon$}

We now investigate the complexity of exactly computing the integrals in \autoref{eqn:psatmain}. We begin with a \PseudoP lower bound for computing $\Vol(\favn)$, and consequently $\psat$ for the uniform parent. We will then discuss lower bounds for non-uniform parents. 

Define the complexity theoretic problem $\PSAT$:
\begin{align}
\label{prob:psat}
 && \PSAT(f,s,d,n) \mapsto \pcon \nonumber \\
\text{Inputs}&:& \text{Parameters of SCS }~ \text{encoding of}~ \fpar, ; s,d \in \Q_+ ; n \in \N \nonumber \\
\text{Output}&:&~ \text{Probability of connectivity}~ \pcon \in \Q_+  
\end{align}

Rational inputs and outputs are specified as exact reduced fractions; for example $s$ is input as the pair $(\num(s),\den(s))$. Let $\PSAT(\Uni)$ denote that subproblem of $\PSAT$ over a uniform SCS.

\begin{theorem}
We have $\Time(\PSAT(\Uni)) \in \Omega(n \log n)$.   
\end{theorem}


Applying \autoref{eqn:psatmain} gives us \cite{KumarTRO2015}
\begin{align}
\label{eqn:pconuni}
\Vol(\ssimpn) = \frac{s^n \cdot \sqrt{n+1} }{ \nor!}, \\ 
\Vol(\unfavn) = \sum_{k=1}^{\nmin} (-1)^{k -1}  \binom{n+1}{k}  
\frac{(s-kd  )^{\nor} \sqrt{\nor +1} }{\nor!}, \\ \nonumber 
\psat = \frac{\Vol(\favn)} {\Vol(\ssimpn)} = 1-\sum_{k=1}^{ \nmin 
} (-1)^{k -1}  \binom{n+1}{k} \big(1- \frac{kd}{s} \big) ^{\nor}. 
\end{align} 

\begin{proof}
\textit{Upper bound:}\label{ub}    \autoref{eqn:pconuni} is a possible 
solution for $\PSAT(\Uni)$; therefore, its worst-case running time forms an upper 
bound for $\PSAT(\Uni)$.  \autoref{eqn:pconuni} runs in $O(\nmin \log n)$ time;  its  
worst-case instances, which have $n > \nmin  $ take $O(n \log n)$ time, 
which forms an upper bound for any solution to $\PSAT$. Note that 
\autoref{eqn:pconuni} forms a \PseudoP algorithm for $\PSAT$. 

\textit{Lower bound:} Consider $\PSAT(\Uni)$ instances with $s = \frac{4}{3}d$, for which 
\begin{align}
\psat = 1 - (n+1)\cdot \frac{1}{4^n} \approx 1- \frac{n}{4^n}
\end{align}

The input size for these instances is $O(\log n)$, but the output size is 
exponential in the input size, implying an $\Omega(n)$ lower bound for any 
algorithm for $\PSAT(\Uni)$. The upper bound of $O(n \log n)$ is off from the lower bound $\Omega(n)$ only by 
a polynomial in the input size of $\PSAT(\Uni)$, implying that algorithms for $\PSAT$ 
consume more time in outputting the solution rather than computing it. The lower bound is an exponential function of the input size,
hence $\PSAT (\Uni) \in \EXP$. 
\end{proof}

\textit{Time Complexity of computing $\Vol(\favn)$}: The $\sqrt{n}$ in the formula for $\Vol(\favn)$ makes it impossible to provide a bounded decimal expansion to $\Vol(\favn)$, 
hence the complexity of writing down $\Vol(\favn)$ is \textit{infinite}, except when $\nor$ is a square.  Remedying this unbounded expansion requires us to compute  $Vol(\favn) \cdot \frac{n!}{\sqrt{n+1}}$, for which the same bounds as $\PSAT(\Uni)$ apply. The same bounds apply to $\Vol(\unfavn) \cdot \frac{n!} {\sqrt{n+1}}$. 


\begin{theorem}
\label{thm:polyint}
 Let $\PSAT(\text{mon})$ denote instances with monomial parents, i.e.  
 \begin{align}
 \fpar(x) := \frac{x^m}{s^{m+1}} \1_{\Bo}
 \end{align}
 for some natural $m$. Then $\Time(\PSAT) = \Theta(n^{m'})$ for some $m' \in \N$.   
\end{theorem}

\begin{proof}
This result follows directly from of the following lemma  \cite{baldoni2011integrate, de2012software,monomialMO}:
\begin{lemma}
 A monomial in $\nor$ variables $\prod \limits_{i=1} ^{n} x_i^{m_i}$ where $m_i \in \N$ can be integrated in $\Poly(\sum m_i)$ time over $\Delta_n$. 
\end{lemma}
\end{proof}

\autoref{thm:polyint} implies  that $\pcon$ can be computed in polynomial time per term for polynomial parents of the form $\fpar (x) = \sum \limits_{0\leq i\leq m} a_i x^{i} \1_{\Bo}$, leading to an overall computation time of $\Theta(m n^{m'})$.  Likewise, the result gives to a \PseudoP complexity for the rescaled Beta pdf 
\begin{align}
\Beta{x}{a}{b}:= Z(a,b) x^{a-1} (s-x)^{b-1} \1_{\Bo} ~\text{where}~ a,b \in \N
\end{align}
which can be decomposed into monomials as
\begin{align}
\label{eqn:betapdf}
 \Beta{x}{a}{b} = Z(a,b) \sum \limits_{k=0} ^{b}  \binom{b}{k} ( x^{a-1} -  x^{a+b-2}) 
\end{align}


\textit{Open cases} To the best of our knowledge, the complexity of $\PSAT(\fpar)$ is open for the following parents:
\begin{enumerate}
\item Beta pdf with rational parameters, with the same form as \autoref{eqn:betapdf} except that $a,b \in \Q_+$. 
 \item Truncated Gaussian $\mathcal{N}(x|\mu,\sigma,a,b)$   
\end{enumerate}

\autoref{tab:iidparents} summarizes all our results. 
\input{Tabs/IID-Parents.tex} 



==> LitRev.tex <==
\section{Related Work}
\label{Sec:LitRev} 





 


==> Noisy.tex <==
\section{Coverage with Noisy Sensors}
\label{Sec:Noisy}
Thus far, we assumed that all robot positions were taken up without any error, and that Wi-fi propagation was threshold-based and propagated only along the line-of-sight (LOS) between two robots. These assumptions are simplistic at best for any experimental scenario. In hindsight, the theory developed in the previous sections, while inapplicable to nonideal scenarios, leads us to our hardness results here.  We will make the following assumptions throughout this section: Robots \textit{intend} to attach to $\Bo$ at predetermined positions, but are prevented from doing so by their noisy odometry and sensing. 


\subsection{Point Robots with Noisy Odometry}
\label{Subsec:mrt-cover}
We illustrate the hardness of determining the properties of robots with noisy odometry using several coverage scenarios.  A team of point robots $\Rob_{1\ldots n}$ jointly chooses the connected position vector  $\posvec_{\text{dest}}$ as per the DCS in \autoref{Subsec:InitAtt}, with $\Rob{i}$ attaching to $\pos{i}$. Subsequently, robots navigate to their positions in increasing order of their ids, travelling at unit speed. Due to noisy odometry, the robot moves as per the SDE:
\begin{align}
 d\upos{i}(t) = 1 + d\Wie_t  \implies \upos{i}(t) = t + \int_{0} ^t d\Wie_s ~ \text{for} ~0 \leq t \leq \pos{i,\text{dest}}) 
\end{align}

where $\Wie_{.}$ is the standard unit-strength Brownian motion. As a result, the error in the final position of $\Rob_{i}$ is given by a normal variate:
\begin{align}
\epsilon_{i}(t) := \upos{i} - \pos{i,\text{dest}} =  \Wie_i \\
E_{i} (t) \sim \mathrm{Nor} (\mu_i = 0, \sigma_i^2 = \pos{i,\text{dest}}).  
\end{align}

In general, the errors are samples of distinct Gaussians; the random error vector $\mathbf{E}$ is a multivariate normal, with zero mean and covariance matrix with diagonal entries $\sigma_i^2$. The  final positions $\posvec + \mathbf{\epsilon}$ are effectively the order statistics of $\mathbf{E}$, which are given by \autoref{thm:bapat}. Consequently, computing the properties of $\G$ are $\PH$, precisely for the same reasons as in \autoref{Subsubsec:renyimpl}.

\subsection{SCS with Partial Observability}
We will make 



\subsection{Wi-fi Localization} \cite{ProakisComm}
\label{Subsec:Wifi}



==> NonUnif.tex <==
\section{Non-uniform i.i.d parents}
\label{Sec:Nonunif}
In this section, we will generalize the uniform i.i.d attachment of \autoref{Sec:Uniform} by replacing a single assumption with a more general version. Each such generalization will lead to an $\NPH$ or $\PH$ problem, prohibiting us from computing $\psat$, or computing saturated pdfs over $\favn$ in $\Poly$ time.  
Let $f(t)$ (resp. $F(t)$) denote the parent pdf (resp. cdf).



\subsection{Piecewise Uniform (PWU) Parents } 



\subsection{Polynomial Parents}



\subsection{Approximating General Functions through Polynomials} 

==> Prelims.tex <==

\begin{comment}
We will now quote standard results from the literature that we will use to prove hardness results in the coming sections. In general, the complexity-theoretic problems will take input in binary encoding, with rational numbers $b \in \Q$ being specified as the fraction $p/q$ in its lowest terms. The size of the input is given by $\size(b) = \size(p) + \size(q) + 1$. When a function with rational inputs needs to output an irrational number of the form $\sqrt{a} \cdot b$, where   $a,b \in \Q$, we will assume that $\sqrt{a}$  is approximated to $\size(b)$ bits. 

\subsection{Order Statistics}
\label{Subsec:ostat}
Suppose we are given samples of $\nor$ random variables $\rvupos{1}$ through $\rvupos{\nor}$. When we sort them in nondecreasing order, we get the variables $\rvpos{1}, \rvpos{2}, \ldots, \rvpos{k},\ldots, \rvpos{\nor}$,  where $\rvpos{k}$ is the $k$-th smallest of the original variables. We call these sorted variables the \textit{order statistics} of the original variables, which are called their \textit{parents} \cite{ostat2003}. When the parents are i.i.d variates with pdf $f(t)$ and $F(t)$, the cdf of the $k$-th order statistic of $\nor$ variables is given by: 
\begin{align}
 F_{T_k} (t) = \sum \limits_{i=k} ^n \binom{n}{i}  F^i(t) (1-F(t))^{n-i}
\end{align}


The joint pdf of order statistics at the indices $\ixs= (n_1,n_2,\ldots,n_k)$, whose entries form a strictly increasing sequence of length not exceeding $n$  is given by :
\begin{align}
\label{eqn:fixs}
 f_{\ixs} (t_1,t_2,\ldots, t_k) = n! \prod \limits_{j=1} ^{k} f(t_j) \prod\limits_{j=0} ^k \frac{{ (F(x_{j+1}) - F(x_j))}^{n_{j+1} - n_j -1}} {(n_{j+1} - n_j -1)!}
\end{align}




\subsection{Volumes of Polyhedra} 
We will use the following results from \cite{DyerFrieze}. Define a \textit{rational halfspace} by the inequality 
\begin{align}
\mathcal{HS}:=\{ \mathbf{x} \in \R^n : \mathbf{a}^T \mathbf{x} \leq b \}, ~ \mathrm{where}~ \mathbf{a} \in \Z_+^n , ~ b \in \mathbb{Q}_+ 
\end{align}
where $\mathbf{a}$  is a vector of strictly positive integers, and $b$ is rational. Let $\genhyp{n}$ be the $n$-dimensional unit hypercube $[0,1]^n$.  Consider the problem $\VOLHSP$, which has inputs of the form $(\mathbf{a}_{1:n}, b)$, consisting of the parameters defining a half-space $\hsp$.  $\VOLHSP$ asks for the volume of intersection  $\Vol( \hsp \cap \genhyp{n})$ as output.

We quote two results from \cite{DyerFrieze, dyer1991computing}:


\begin{theorem}
\label{thm:phard1}
$\VOLHSP$ is $\PH$.    Equivalently, it is $\PH$ to compute the probability that a uniform pdf over a hypercube satisfies a single linear inequality.
\cite{dyer1991computing}
%\begin{align}
 %\hsp \cap \hyp{n} %:= \{ \mathbf{x} \in \R^n : \0_n \leq \mathbf{x} \leq \1_n \wedge \mathbf{a}^T \mathbf{x} \leq b \}.
 %\end{align}

 
\end{theorem}

\cite{DyerFrieze} derives this result by reducing the counting knapsack problem $\#\KNAP(\mathbf{a}, b)$ to $\VOLHSP$.   $\#\KNAP(\mathbf{a},b)$ asks for the number of ways to place  the weights  $a_i \in \mathbf{a}$ into a  knapsack, without exceeding its capacity $b$. Let $\favn := \hsp \cap \genhyp{n}$. From \cite{dyer1991computing}, we may express $\favn$ as the intersection of overlapping simplices by
\begin{align}
\label{eqn:overfavn}
\favn = \{ \forall ~\mathbf{v} \in \vm(\genhyp{n}): \bigcap \gensimp (\mathbf{v}) \}.  
\end{align}

Here $\gensimp(\mathbf{v})$ is a simplex with vertices 
\begin{align}
\label{eqn:simpv} 
 \vm(\gensimp(v)) = \begin{bmatrix} \mathbf{v} & \mathbf{v} - \frac{b-\mathbf{a}^T \mathbf{v}}{a_1} \mathbf{e}_1   & \ldots &  \mathbf{v} - \frac{b-\mathbf{a}^T \mathbf{v}}{a_n} \mathbf{e}_n \end{bmatrix}.   
\end{align}


Since these simplices overlap, $\Vol(\favn)$ needs to be determined by the Inclusion-Exclusion Principle (IEP). Noting that
\begin{align}
 \Vol(\gensimp(v)) = \frac{n!}{\prod_{i=1}^n a_i} \max(0,b - \mathbf{a}^T\mathbf{v} )^n    
\end{align}

we have

\begin{align}
\label{eqn:volhsp}
 \Vol(\favn) = \sum \limits_{\mathbf{v} \in \vm(\genhyp{n}) } (-1)^{\1^T \mathbf{v}} \Vol(\gensimp(\mathbf{v})).  
\end{align}


Note that the exponent of $-1$ is the number of ones in $\mathbf{v}$.  The sum in \autoref{eqn:volhsp} is taken over all vertices of $\genhyp{n}$, with only those vertices within $\hsp$ contributing to it; the contribution of exterior vertices is set to $0$ by the $\max{}$ function. We have in addition the hardness results: 
\begin{theorem}
 \label{thm:phard2}
 Computing the quantity
 \begin{align}
 Q(b):= \sum \limits_{\mathbf{x} \in \vm(\genhyp{n}) } (-1)^{\1^T \mathbf{x}}  { (\max(b-\mathbf{a}^T \mathbf{x}),0))^{n} } 
 \end{align}

 is  (a) $\PH$ when $\mathbf{a}$ and $b$ are unrestricted \cite{DyerFrieze}, and (b) $\NPH$ when $\mathbf{a}$ and $b$ have polynomial size in $\nor$ \cite{khachiyan1993complexity}. 
 
\end{theorem}




\begin{theorem}
Given $m$ rational vectors $\mathbf{x}_1, \ldots, \mathbf{x}_n$ each of length $\nor$.  It is $\PH$ to compute the volume of their convex hull $\mathrm{conv} (\mathbf{x}_1,\ldots, \mathbf{x}_n)$. 
\end{theorem}


\subsection{Integration over Simplices}

%Define a \textit{linear form} of a vector $\mathbf{x} \in \R^n$ as one of the form $\mathbf{a}^T \mathbf{x}$ \cite{baldoni2011integrate}. For our purposes, the coefficient vector $\mathbf{a}$ is rational. 

Let $\gensimp_D$ denote the full-dimensional simplex 
\begin{align}
\label{eqn:fullsimp}
\gensimp_D = \{\mathbf{x} \in \R^{D} : \mathbf{x} \geq \0, ~\text{and}~ \1^T \mathbf{x} \leq 1 \}. 
\end{align}

All our polynomials will be functions of the form $g(\mathbf{x}) = g(x_1,x_2,\ldots,x_n)$, with rational coefficients, and fully paranthesized. For our purposes, we may suppose that $g$ is represented as a fully paranthesized expression involving the operators $+,-,$ and $\times$. Define the problem $\INTSIMP$ which takes inputs  $(d,g,\bitpos)$ where $d$ and $g$ are as defined above, and $\bitpos$ is a nonnegative integer denoting a bit position in the output. $\INTSIMP$ asks for the bit at position $\bitpos$ of 
\begin{align}
I(g,\gensimp_D) = \int_{\mathbf{x} \in \gensimp_D} g(\mathbf{x}) d\mathbf{x}.
\end{align}

From \cite{baldoni2011integrate, lasserre2001multi}, we have the results: 

\begin{theorem}
\label{thm:intsimp}
$\INTSIMP$ is (a) $\NPH$ if $g(\mathbf{x})$ is unrestricted ,(b) $\Poly$ if the degree of $g$ is bounded,  and (c) $\Poly$ if the number of variables involved in $g(\mathbf{x})$ is bounded. 
\end{theorem}

We may rewrite \autoref{eqn:fullsimp} to change the inequality $\1^\mathbf{x} \leq 1$ into an equation, thereby making it a degenerate polytope in $\R^{D+1}$, as:
\begin{align}
\label{eqn:degsimpn}
 \gensimp_D = \{\mathbf{x} \in \R^{D+1} : \mathbf{x} \geq \0, ~\text{and}~ \1^T \mathbf{x} = 1  \}.
\end{align}

The coordinates $(x_1,\ldots,x_{n+1})$ are the barycentric coordinates of points in $\gensimp_D$. Let  $\gensimp(\vvec_{1:D+1})$ denote the $D$-dimensional simplex with vertices at $\vvec_{i}$, i.e. one with vertex matrix
\begin{align}
 \vm(\gensimp) = \begin{bmatrix} \vvec_1 & \ldots & \vvec_{D+1} \end{bmatrix}.
\end{align}



An arbitrary point within this simplex is expressible in barycentric form as 
\begin{align}
\mathbf{x}^T  \vm (\gensimp) = \sum_{i=1} ^{n+1} x_i \vvec_i, ~\text{where}~ \mathbf{x}_{1:n+1} \geq \0, ~\text{and} ~ \1^T \mathbf{x} = 1. 
\end{align}

Now we define the following exponential notation for vectors. Given the generic vector $\mathbf{y} \in \R^n$, and a vector of nonnegative exponents $\exps = (m_1,\ldots,m_n) \in \mathbb{Z}_{\geq 0} ^n$ \textit{same length} as $\mathbf{y}$, define   
\begin{align}
\label{eqn:exps2}
 \mathbf{y} ^{\exps} := y_1 ^{m_1} \cdot y_2 ^{m_2} \ldots \cdot y_n^{m_n}. 
\end{align}


\end{comment}




==> Renyi-App.tex <==
\subsection{Applications and Extensions}
\label{Subsec:Renyi-App}
The reduction in the previous section 

\subsubsection{Polynomials of arbitrary degree}


\subsubsection{Linear Transformations of order statistics}







